Automated Discovery of Functional Actual Causes in Complex Environments

Reinforcement learning (RL) algorithms often struggle to learn policies that generalize to novel situations due to issues such as causal confusion, overfitting to irrelevant factors, and failure to isolate control of state factors. These issues stem from a common source: a failure to accurately identify and exploit state-specific causal relationships in the environment. While some prior works in RL aim to identify these relationships explicitly, they rely on informal domain-specific heuristics such as spatial and temporal proximity. Actual causality offers a principled and general framework for determining the causes of particular events. However, existing definitions of actual cause often attribute causality to a large number of events, even if many of them rarely influence the outcome. Prior work on actual causality proposes normality as a solution to this problem, but its existing implementations are challenging to scale to complex and continuous-valued RL environments. This paper introduces functional actual cause (FAC), a framework that uses context-specific independencies in the environment to restrict the set of actual causes. We additionally introduce Joint Optimization for Actual Cause Inference (JACI), an algorithm that learns from observational data to infer functional actual causes. We demonstrate empirically that FAC agrees with known results on a suite of examples from the actual causality literature, and JACI identifies actual causes with significantly higher accuracy than existing heuristic methods in a set of complex, continuous-valued environments.

==> sections/broader-impact.tex <==
\section{Broader Impact}

Context-specific reasoning and the ability to infer actual causes can be used to improve the performance and robustness of decision-making systems, and this is the application we focus on in this paper. The long-term impact of high-performing autonomous agents, both negative and positive, is a shared concern across much of RL research. In addition to this, tractable algorithms for inferring actual causes from data, including JACI, may have an impact in applications such as blame attribution, safety evaluation, and explanation in AI systems, and offer valuable insights into actual causes of model behavior for research in AI alignment. 

Prior work on actual causation in philosophy has taken inspiration from problem settings related to legal judgments, and as the field advances toward real-world domains and data-driven inference, it is natural that attention may return to such problem settings. Capabilities such as tracing the sequence of events that led to an agent's decision or outcome are key to closing the gap between public policy and the rapid progress of black-box AI systems. 

However, given that many potential applications for automated inference of actual causes are related to judgments and accurate decision-making, many of the risks associated with them are related to automation bias \cite{mosier2017automation}. This refers not only to placing undue trust in models and their conclusions, but also implicitly to how they were trained and the biases that they can perpetuate \cite{angwin2022machine}. To this end, we encourage further research and discussion on:

\begin{itemize}
    \item Assumptions about norms or human judgments that underlie different methods of inferring actual causes.
    \item Identification of ground truth actual causes for empirical evaluation with real-world data or human annotations, and how this differs between applications that can involve subjective judgments (e.g. explanation, blame attribution) and less subjective applications (e.g. interaction detection in physics simulators).
\end{itemize}
